VINP: Variational Bayesian Inference with Neural Speech Prior for Joint ASR-Effective Speech Dereverberation and Blind RIR Identification

Reverberant speech, denoting the speech signal degraded by reverberation, contains crucial knowledge of both anechoic source speech and room impulse response (RIR). This work proposes a variational Bayesian inference (VBI) framework with neural speech prior (VINP) for joint speech dereverberation and blind RIR identification. In VINP, a probabilistic signal model is constructed in the time-frequency (T-F) domain based on convolution transfer function (CTF) approximation. For the first time, we propose using an arbitrary discriminative dereverberation deep neural network (DNN) to estimate the prior distribution of anechoic speech within a probabilistic model. By integrating both reverberant speech and the anechoic speech prior, VINP yields the maximum a posteriori (MAP) and maximum likelihood (ML) estimations of the anechoic speech spectrum and CTF filter, respectively. After simple transformations, the waveforms of anechoic speech and RIR are estimated. VINP is effective for automatic speech recognition (ASR) systems, which sets it apart from most deep learning (DL)-based single-channel dereverberation approaches. Experiments on single-channel speech dereverberation demonstrate that VINP attains state-of-the-art (SOTA) performance in mean opinion score (MOS) and word error rate (WER). For blind RIR identification, experiments demonstrate that VINP achieves SOTA performance in estimating reverberation time at 60 dB (RT60) and advanced performance in direct-to-reverberation ratio (DRR) estimation. Codes and audio samples are available online.

==> responses/R1.tex <==
\begin{answerreviewer}[AQ - Publish With Minor, Required Changes]

\qa{Improve the writing by removing slight repetitions and enhancing coherence in the Introduction and Method sections.}
{Thanks for your advice. We have revised the expression.}

\qa{Provide a more detailed justification for the selection of DNN architectures used within VINP.}
{Both DNNs are representative approaches in dereverberation.
TCN+SA+S includes a self-attention module to produce dynamic representations given input features, a temporal convolutional network (TCN) to learn a nonlinear mapping from such representations to the magnitude spectrum of anechoic speech, and a 1-D convolution module to smooth the enhanced magnitude among adjacent frames.
Different from TCN+SA+S, oSpatialNet-Mamba employs a 1-D convolution input layer and a linear output layer, and the so-called stacked cross-band and narrow-band blocks to build a mapping between complex-valued spectrums.
The narrow-band block, composed of self-attention layers and convolutional layers along the time axis, processes each frequency independently with the same network parameters.
The cross-band block, composed of convolutional layers along the frequency axis and full-band linear modules, processes each frame independently with the same network parameters.
We use VINP-TCN+SA+S and VINP-oSpatialNet to demonstrate the performance of two DNNs with different architectures and capabilities in the tasks of dereverberation and blind RIR identification.
We have clearfied it in \refcm{selectbackbone}.}


\qa{Explain the rationale behind the choice of 100 iterations for the VBI process and whether adaptive stopping was considered.}
{
As shown in Fig. \ref{fig:CurveDereverb} and Fig. \ref{fig:CurveRIR}, some metrics such as likelihood, PESQ and MAE of RT60 get better as the iteration continues, whereas ESTOI, DNSMOS, WER and MAE of DRR seem to converge after several iterations.
Therefore, the number of iterations should take into account both the computing power and the objective and we did not use adaptive stopping.
We think that for speech dereverberation, 100 iterations are sufficient to achieve satisfactory human perception and ASR performance, with limited gains from additional iterations.
And for RT60 estimation, more than 300 iterations can be considered.
We have added the expression of the stopping rule in \refcm{stoprule}.
We will consider adaptive stopping rules in our future work.}

\qa{VINP assumes stationary noise, which may not cover all real-world situations. It would be better if they at least briefly discussed the limitations of this assumption.}
{Thanks for your advice. 
Because VINP is a dereverberation method developed based on a stationary noise model, we don't recommend using it in overly complex noisy environments.
Therefore, the training dataset contains only stationary noise, and we cannot directly use it on nonstationary noise.
However, it is possible to analyze the effect of unstationary noise on VEM using the oracle anechoic prior.
Therefore, we added a discussion under different noise conditions in \refcm{noiseExp}, including lower SNR and non-stationary noise.
Compared to the results with stationary noise, dereverberation performance using an oracle prior shows degradation under mismatched non-stationary noise conditions, particularly at low SNRs.
}


\end{answerreviewer}

==> responses/R2.tex <==
\begin{answerreviewer}[RQ - Review Again After Major Changes]

\qa{The experimental setup lacks details about recording equipment. Could you explicitly specify: Microphone models/specifications used for capturing test samples; Speaker types/positions in simulated environments; Acoustic treatment of experimental spaces (if any real recordings were made)?}
{The training utterances are generated by convolving source speech with reverberant and direct-path RIRs, followed by noise addition.
The source speech consists of 200 hours of high-quality English speech utterances, including the utterances in DNS Challenge and VCTK that have a raw DNSMOS p.835 score exceeding 3.5, as well as the whole EARS corpus.
We simulate 100,000 pairs of reverberant and direct-path RIRs using the gpuRIR toolbox.
The simulated speaker and omnidirectional microphone are randomly placed in rooms with dimensions randomly selected within a range of 3 m to 15 m for length and width, and 2.5 m to 6 m for height.
The minimum distance between the speaker/microphone and the wall is 1 m. 
Reverberant RIRs have RT60 values uniformly selected within the range of 0.2 s to 1.5 s. 
Direct-path RIRs are generated using the same geometric parameters as the reverberant ones but with an absorption coefficient of 0.99.
Noise recordings from NOISEX-92 and the training set of REVERB Challenge are used.
The SNR is randomly selected within the range of 5 dB to 20 dB.

For speech dereverberation, we utilize the official single-channel test set from the REVERB Challenge, which includes both simulated data (marked as 'SimData') and real recordings (marked as 'RealData').
In SimData, there exist six distinct reverberation conditions: three room volumes (small, medium, and large), and two distances between the speaker and the microphone (50 cm and 200 cm). The RT60 values are approximately 0.25 s, 0.5 s, and 0.7 s. 
The noise is stationary, mainly generated by air conditioning systems. 
SimData has a SNR of 20 dB.
RealData consists of utterances spoken by human speakers in a noisy and reverberant meeting room. It includes two reverberation conditions: one room and two distances between the speaker and the microphone array (approximately 100 cm and 250 cm). The RT60 is about 0.7 s.


For blind RIR identification, a test set named 'SimACE' is constructed.
In SimACE, microphone signals are simulated by convolving the clean speech from the 'si\_et\_05' subset in WSJ0 corpus with the downsampled recorded RIRs from the 'Single' subset in ACE Challenge, and adding noise from the test set in REVERB Challenge.
The minimum and maximum RT60s are 0.332~s and 1.22 s, respectively.
More details about the RIRs can be found in.
SimACE has a SNR of 20 dB.

We clarified the relevant settings in Section IV A.
For more details, please see the original papers of the datasets.
One can use our open-source codes to generate the same training data.
}

\qa{While Section IV-B1 mentions STFT parameters, the core sampling rate (16kHz/48kHz?) for processing isn't explicitly stated. Please confirm whether all experiments used consistent sampling rates.
}{ 
The sampling rate is 16kHz. We emphasized the sampling rate in Section IV-A and Section IV-B1.}

\qa{The paper mentions using "stationary background noise." To ensure generalizability: What specific noise categories were included?Were transient noises considered? How does performance vary with non-Gaussian noise distributions?}
{Stationary noise follows the definition of a stationary random signal. 
In our test set, the noise is mainly generated by air conditioning systems, as shown in Section IV A.
% That means, the noise is real-recorded rather than Gaussian.
% The Gaussian prior of noise is for simplicity in derivation.

We replaced the noise in REVERB SimData and SimACE with the noise from CHiME4, which was collected from four distinct environments: buses, cafes, pedestrian zones, and street intersections.
The transient noise is included.
Compared to the results with stationary noise, dereverberation performance using an oracle prior shows degradation under mismatched non-stationary noise conditions, particularly at low SNRs.
Please see \refcm{noiseExp}.
}

\qa{What RMS error levels exist between CTF approximation vs. full convolution? Are there comparative results using alternative models (e.g., WPE)?}
{
In \refcm{CTF}, we added the references that analyze the error level of CTF approximation theoretically and experimentally.
The RIR reconstruction errors using CTF approximation are below -20dB.
For more details, please see \textit{Tang et. al., Personal sound zones in the short-time Fourier transformdomain with relaxed reverberation. 
https://doi.org/10.1121/10.0035578}

CTF is the representation of reverberation in the T-F domain, whereas WPE is a linear prediction-based dereverberation method.
WPE can be implemented in both time domain with full convolution and in T-F domain with CTF approximation.
It is reported that using full convolution in WPE is better than CTF approximation, as in \textit{Rosenbaum et. al., Crossband Filtering for Weighted Prediction Error-Based Speech Dereverberation. https://doi.org/10.3390/app13179537}.
In our experiments, we use the WPE in the time domain, which corresponds to the full convolution.
}

\qa{The VBI program in VINP can be executed in parallel across T-F bins, and the final detection indicators MAE and RMSE are time-domain indicators. Would you like to consider adding some frequency-domain indicators, such as LSD?
}{
We added the LSD metric in Table \ref{tab:results_SD}.
Although the LSD does not match the perception quality and ASR performance, we employ it to demonstrate the magnitude spectrum restoration capability of VEM.
}

\qa{Is there any basis for mentioning in the introduction that "the convolution transfer function (CTF) approximation is a rather accurate model of the reverberation effect" as a theoretical support for the algorithm? Are there references or other experiments to prove it?}{
In \refcm{CTF}, we added the references that analyze the error level of CTF approximation theoretically and experimentally.
}

\qa{What architectural modifications make oSpatialNet more ASR-effective? Do their computational profiles differ significantly? Is there a performance tradeoff between them in low-reverberation vs. high-reverberation conditions?
}{
% It remains challenging to determine the effect of front-end network structure on back-end tasks. 

The effectiveness of oSpatialNet for ASR tasks may be attributed to its narrow-band processing mechanism, namely processing frequencies independently.
Because narrow-band processing is especially efficient for modeling the narrow-band room filter convolution and narrow-band processing can avoid the so-called wide-band artifacts, such as the blurred and/or wrongly deleted/inserted wide-band spectra, which will be very harmful for ASR. In the revised manuscript, we have added reference paper for this analysis, please see \refcm{selectbackbone}.


We demonstrate the PESQ for 3 rooms with different RT60s in REVERB Challenge. There doesn't seem to be any obvious trade-off between low-reverberation and high-reverberation conditions.
\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c}
         Method&Room1 (RT60=0.25s)&Room2(RT60=0.5s)&Room3(RT60=0.7s)  \\
         \hline
         Unprocessed&1.87&1.30&1.27\\
         VINP-TCN+SA+S&2.78&2.46&2.31\\
         VINP-oSpatialNet&3.12&2.66&2.69\\
    \end{tabular}
\end{table}}



\qa{For practical deployment: What is the worst-case processing latency per 1-sec utterance? Have you tested on embedded platforms? Does parallelization actually achieve linear speedup with core count?}
{VINP is an offline framework. 
Using 100 iterations, the RTF on NVIDIA A100 is about 2.5.

We did not test it on embedded platforms.

The parallelization achieves linear speedup with core count when the number of cores is less than FT in our manuscript, because the computations are conducted in parallel across T-F bins. 
In practice, we use the vmap function in Pytorch for vectorized implementation across batch dimensions.
}

\qa{ How does performance degrade with moving speakers? Is there a tracking mechanism for gradual acoustic changes?}{
Unfortunately, the current framework cannot handle the moving speakers. 
% It is possible to modify the signal model to do this. 
% This is because for mobile speakers, the CTF filter is time-variant, which greatly increases the number of unknown parameters. 
We will consider this topic in our future work.}

\qa{What performance loss occurs at 0dB SNR? Have you tested with non-stationary noise? Does the method fail catastrophically under impulsive noise?}{
We added a discussion under different noise conditions in \refcm{noiseExp}, including lower SNR and non-stationary noise.
% We found that VINP does not fail catastrophically under mismatched noise conditions.
Compared to the results with stationary noise, dereverberation performance using an oracle prior shows degradation under mismatched non-stationary noise conditions, particularly at low SNRs.
}

\end{answerreviewer}

==> responses/R3.tex <==
\begin{answerreviewer}[RQ - Review Again After Major Changes]
\qa{I am surprised that some of the "SOTA" baselines perform worse than the reported discriminative baselines. I believe the authors made a good effort to ensure a fair comparison, but the results are still unexpected.
In my opinion, the most interesting comparison is between the proposed VINP variants and their corresponding discriminative models. An improvement here would directly justify the method. However, the fact that oSpatialNet outperforms VINP-oSpatialNet on speech dereverberation metrics is a negative result.
}{We have retrained all comparison methods using the latest official releases of both the comparison methods and ASR models.
For all implementations, we utilized the same training set.
All comparison methods were trained until overfitting occurred.
Thus, this should constitute a fair comparison.
The new results are presented in Table \ref{tab:results_SD}. In addition, we have also added two new metrics, i.e. subjective MOS and LSD.
Subjective listening tests show that MOS scores of VINP and StoRM are obviously higher than the other approaches including oSpatialNet*, indicating the limitations of PESQ and DNSMOS as evaluation metrics for the present work.
Analysis in detail is shown in \refcm{listeningtest}.
}


\qa{VINP-TCN+SA+S does show improvement over its discriminative baseline, suggesting that VINP improves performance when the underlying discriminative model is less capable. I understand that TCN+SA+S may be hindered by the use of a phase retrieval algorithm, which could partly explain the benefit of using VINP.

I do see the potential advantages of VINP as illustrated in Figure 5, but it is hard to assess fairly since the comparison between VINP and its base model is not perfectly aligned. Specifically:

1- Why not include a spectrogram-domain metric for a fairer comparison, especially given the reliance on magnitude-only estimation?

2- Alternatively, use a state-of-the-art model for spectrogram inversion to assess whether VINP’s improvements are merely due to better waveform reconstruction.

3- Also, VINP-oSpatialNet should be compared against the same oSpatialNet model used to provide the prior, not a modified version adapted for complex-valued spectrum prediction.}
{
Thanks for your suggestions.

1. We added the LSD metric in Table \ref{tab:results_SD}, which quantifies the similarity between spectrograms.

2. An advanced spectrogram inversion method, i.e. Griffin-Lim’s iterative algorithm, was actually used in the original paper of TCN+SA+S.
Therefore, we have also used it to eliminate potential controversies.


3. We add the comparison between VINP with and without VEM in Table \ref{tab:results_SD}. 
In VINP w/o VEM, we use only the DNNs to enhance the speech magnitude spectrum and keep the phase spectrum reverberant, resulting in a spectrum as $|{\hat{\mathbf{S}}}_{\mathrm{N}}|\exp{(j \angle \mathbf{X)}}$.
Here you can observe how the modification of DNN and VEM iterations impact various metrics of the speech signal.
The difference of LSD between VINP and VINP w/o VEM indicates that VEM brings improvements to the magnitude spectrum.
}

\qa{Please include statistical significance testing for key paired comparisons (e.g., VINP vs. its discriminative baseline). This is essential to validate whether the observed improvements are meaningful.}
{We added Z-testing results for WERs between VINP-oSpatialNet and oSpatialNet*, as well as VINP-TCN+SA+S and TCN+SA+S because the WERs of these methods with 'small' and 'medium' Whisper models are close. 
Results indicate that all differences are significant with $p<0.05$, except for VINP-oSpatialNet and oSpatialNet* on the Whisper ’medium’ model. Please see \refcm{Ztest}. 
}

\qa{Page 10, line 34: The phrase “In subjective evaluation…” is misleading. DNSMOS is an objective metric, even if it is trained to approximate subjective scores.
→ If the authors claim VINP exhibits a higher degree of naturalness, I would strongly recommend conducting a formal subjective listening test to verify this. If successful, this would significantly strengthen the evaluation. Otherwise, the benefit of VINP appears to lie mainly in blind RIR estimation.}
{Thanks for your advice. We have modified the statement. 
A subjective listening test was added in the revised manuscript in Table \ref{tab:results_SD}, which confirmed the advantage of VINP in terms of speech quality.
Additionally, we encourage the readers to access the audio examples online for direct evaluation.
}

\qa{I understand that BUDDy, being unsupervised, does not suffer from generalization issues related to RIRs. However, it still depends on the clean speech corpus used during training. Therefore, the comparison is not entirely fair unless BUDDy is retrained using the same set of dry utterances used to train TCN+SA+S and oSpatialNet. That said, I recognize that retraining BUDDy may be technically challenging, and in such cases, using a publicly available pre-trained model is a reasonable compromise. Nevertheless, BUDDy is the only recent baseline included for blind RIR estimation, and I do not believe it is sufficient to support the claims made. In particular, there exist supervised deep learning approaches for blind RIR or room parameter estimation that could serve as relevant additional baselines. Including at least one such method would significantly strengthen the evaluation.}
{
Yes, the retraining of BUDDy is challenging and we use the pre-trained model.
However, your concern is valid.
Therefore, we also included the well-known FiNS trained on the same dataset for RIR identification.
Please see Table \ref{tab:RIR_estimation}.
}


\qa{In addition, I would suggest considering two more baselines to contextualize the contributions of VINP:

- Oracle-based CTF optimization: Using the oracle (ground-truth) dry speech to directly optimize the CTF parameters would help expose potential limitations of the CTF approximation itself.

- Two-stage inference baseline: Use the anechoic speech estimate from the discriminative model and then optimize only the RIR while keeping the speech fixed. This would allow the authors to isolate and highlight the benefits of VINP’s joint inference framework over simpler sequential approaches.
}{
We added the discussion in \refcm{noiseExp}. We used the oracle anechoic speech prior to isolate the influence of DNNs and discussed the limitations of VEM itself.


VEM updates the posterior of speech and CTF filter in E-step and M-step iteratively and jointly.
If we fix the E-step, $\mathbf{H}$ will be updated in M-step only once.
If we use the anechoic speech estimate from a discriminative DNN as the mean of the posterior, the CTF filter will be estimated by least-squares according to Eq. (\ref{eq:est_H}).
Using the output of the original TCN+SA+S, and also using clean speech for reference, as the mean of the posterior, the MAE of RT60 estimation is shown as follows. It seems that it is not proper to use the estimated anechoic speech of TCN+SA+S for further estimating RIR based on least-squares, possibly due to the distortion of enhanced speech. 

\begin{table}[H]
    \centering
    \begin{tabular}{c|c}
         Methods&MAE of RT60 (s)  \\
         \Xhline{1PT}
         VINP-TCN+SA+S&0.089\\
         VINP-TCN+SA+S (fixed TCN+SA+S output)&0.867\\
         VINP (fixed clean speech)&0.067
    \end{tabular}
\end{table}





% We cannot fix the speech and optimize only the RIR for two reasons:

% 1) Fixed speech estimate means a fixed E-step, and the RIR will be updated in M-step only once.

% 2) The estimation of anechoic speech corresponds to its posterior mean. 
% While we can fix the posterior mean during iterations, it remains challenging to determine a reasonable posterior variance.
}

\qa{"The anechoic speech, often regarded as an oracle, serves as the ultimate target of speech dereverberation."
It’s unclear what "oracle" means in this context. Please clarify.}
{We revised the expression. Currently, we use the expressions of 'oracle prior' and 'clean/anechoic speech'.}

\qa{"there is a strong need to estimate the anechoic speech and RIR"
Please describe specific applications where this is needed (e.g., far-field ASR, virtual acoustics, speech enhancement, audio forensics).}{We added it in \refcm{rirapplications}.}

\qa{page 3, line 16
"Analyzing and processing speech signals in the time domain poses significant challenges."
Please briefly specify these challenges, or cite a relevant reference.}
{This is clarified in the revised manuscript, see \refcm{RIR_long}. The challenge lies in the estimation of the very long time-domain RIR filter (normally thousands of taps). 
For example, the estimation of filter, e.g. Eq.~(\ref{eq:est_H}) in the proposed method, shares similar solutions in T-F domain and time domain.
But the solution in time domain requires the inversion of a very large correlation matrix, which suffers from very high computational/memory costs and poor robustness.
}

\qa{After Eq. 2
It would be helpful to state explicitly why the CTF is an approximation (e.g., it omits inter-band STFT correlations).}
{This is clarified in the revised manuscript, see \refcm{CTF}. In addition, we added the references that analyze the error level of CTF approximation theoretically and experimentally.}

\qa{I understand the assumption and its role in the formulation, but it’s not entirely true in practice. A DNN trained on speech naturally captures T-F dependencies, so assuming full independence across T-F bins seems questionable. Could you please comment on this?
}{These assumptions are applied to the priors of anechoic speech and noise, which only affect the subsequent VEM rather than DNN training. 
% The choice of prior in Bayesian inference is subjective. 
In our work, we use a T-F independent prior assumption to balance rationality and computational feasibility. 
% The theoretical basis is that the correlation of speech samples decreases as the time interval increases. 
Although this assumption may differ from reality, it is a compromise to obtain a closed-form solution. Additionally, while the speech prior is assumed to be T-F independent, the ideal posterior distribution of anechoic speech given the observed data is not T-F independent, which aligns with reality. This is clarified in the revised manuscript, see \refcm{dependency}.
}

\qa{Eq. 14
The KL divergence-based loss is reasonable. However, it would be good to compare it in the evaluation against a standard objective such as MSE to show its benefit.}
{Such a loss function is different from that in regular discriminative dereverberation DNNs which directly predict the anechoic spectrum, but shares the same formula with Itakura-Saito divergence between power spectra, which is widely used in VAE-based unsupervised speech enhancement approaches.
We have also explored various loss functions, including MSE and MAE for linear and logarithmic spectra, alongside backward KL divergence. Experimental results confirm that KL loss is a better choice in the proposed VINP framework. 
Using MSE, the dereverberation performance on REVERB SimData is
\begin{table}[H]
    \centering
    \begin{tabular}{c|c|c}
         Method&PESQ&DNSMOS P.835  \\
         \Xhline{1pt}
         VINP-TCN+SA+S&2.52&3.10\\
         VINP-TCN+SA+S (MSE loss)&2.33&2.88
    \end{tabular}
\end{table}
% Due to space limitations, we do not show these experiments in the manuscript.
We have clarified this in \refcm{lossfunc}.
}

\qa{Eq. 18.
This is just a notation choice. But I think
The model parameters $\theta$ should be incorporated in the joint density p(S,X) somehow, either as $p_\theta(S, X)$, or $p(S, X; \theta)$. The same applies in Eq. 9, where the CTF $\mathbf{H}$ is not reflected into the joint density.}{We have modified almost all formulas according to your suggestion.}

\qa{Eq. 28.
$\alpha$ was previously defined using Eq 12 based on the DNN output, and it is mentioned that this variable is kept fixed. Why is it initialized differently here? This might be a typo or oversight.}{This typo was fixed.}

\qa{Section 3.C.
The approach looks valid overall.
However, I don't fully understand why it is necessary to use the pseudo-measurement process insteadn of simply applying iSTFT to H. To my understanding, H represents the STFT of the time-domain RIR.
I would guess the authors do this to be consistent with the CTF approximation and obtain a time-domain representation that exactly matches the forward model. It would be helpful to clarify this explicitly. Why is iSTFT of H alone not sufficient in practice?}
{
CTF is not the STFT of RIR, but the model of reverberation in the T-F domain.
That means we have $x(n)=h(n)*s(n)$ and $\mathrm{istft}(X(f,t))\approx \mathrm{istft}(\sum_{l=0}^{L-1}H_l(f)S(f,t-l))$, but $\mathrm{istft}(H_l(f)) \neq h(n)$.
To the best of our knowledge, there exists no closed-form transformation that can convert CTF filters to RIR directly.
Therefore, according to the signal model, we simulate the measurement process in real-world to get the STFT of pseudo observation signal. 

We are not sure whether iSTFT is sufficiently effective. We also test the iSTFT of H, and the MAE of RT60 estimation is shown as follows. It seems that a plain application of iSTFT does not work well for our case, and further research on this issue may be needed. 
\begin{table}[H]
    \centering
    \begin{tabular}{c|c}
         Method&MAE of RT60 (s)\\
         \Xhline{1pt}
         VINP-TCN+SA+S& 0.089 \\
         VINP-TCN+SA+S (iSTFT)&0.219 
    \end{tabular}
\end{table}
}


\qa{Section 4.
I understand that oSpatialNet is originally designed for multichannel signals. However, this paper focuses on single-channel. How is oSpatialNet adapted for the single-channel case? The use of "Spatial layers" in Fig. 3(b) is confusing and not clearly explained.}{
oSpatialNet was initially proposed for multi-channel applications. 
However, as shown by the single-channel ablation experiment provided in the original SpatialNet paper [r1] and by more single-channel experiments and analyses provided in a subsequent paper [r2], SpatialNet (and oSpatialNet) is able to achieve promising results as well when directly used for single-channel applications. One major reason is that SpatialNet can still learn/leverage spatial information, i.e. the (single-channel) RIR/CTF-modelling of speech, for conducting speech dereverberation. 
% The narrow-band block, designed based on CTF approximation, is able to learn such spatial information and remove narrow-band noise, thereby enabling single-channel speech dereverberation.
% Subsequent research has evaluated its effectiveness in single-channel speech processing tasks by modifying the number of input channels.
In the revised manuscript, we have further clarified this issue, please see \refcm{selectbackbone}. 

Expression of 'Spatial layers' has been removed.

[r1] Changsheng Quan, Xiaofei Li. SpatialNet: Extensively Learning Spatial Information for Multichannel Joint Speech Separation, Denoising and Dereverberation. IEEE/ACM TASLP, 2024.

[r2] Nian Shao, et al. Cleanmel: Mel-spectrogram enhancement for improving both speech
quality and ASR. IEEE TASLPRO, 2025.
}

\end{answerreviewer}

==> responses/coverletter.tex <==
\begin{coverletter}{VINP: Variational Bayesian Inference with Neural Speech Prior for Joint ASR-Effective Speech Dereverberation and Blind RIR Identification}{T-ASL-11563-2025}
\begin{answereditor}{Based on the enclosed set of reviews, your manuscript requires a MAJOR REVISION (RQ). In particular there are concerns about the experimental part.}
We would like to express our sincere gratitude to the reviewers and editor for their comments, which are helpful in improving the quality of our manuscript. 

Based on the reviewers' comments, we have revised our manuscript as follows:

\textbf{Major revisions:}
\begin{itemize}
 \item The results in Section \ref{sec:expset} were updated. More metrics were employed, including MOS and LSD.
 Notice that in the revised manuscript, we use the overall score of DNSMOS P.835 rather than the raw overall score.
 \item We added a discussion on the performance of VEM algorithm under various noise conditions, including lower SNR and non-stationary noise.
\end{itemize}

\textbf{Minor revisions:}
\begin{itemize}
 \item The typos were fixed. The writing was improved.
 \item The writing style of almost all formulas was modified according to the suggestion of Reviewer 3.
\end{itemize}

We took care to address all the concerns of the reviewers. Please find below our detailed answers to the reviewers' questions and comments.
A revised manuscript is attached after the cover letter, in which the major revisions are highlighted. 

\end{answereditor}

\input{responses/R1}
\input{responses/R2}
\input{responses/R3}


\end{coverletter}

\twocolumn
\setcounter{page}{1}
\setcounter{figure}{0}

==> sections/2.Related.tex <==
\section{Related Works}
\label{sec:related_works}
% Our 





% Introduce several speech enhancement and dereverberation methods based on DNN and Bayesian inference.

% VAE-NMF~\cite{baby2021speech}

% DVAE-VEM~\cite{bie2022unsupervised}

RVAE-EM~\cite{wang2024rvae}
The cubical increase in computation with input length addresses a major limitation observed in our previous publication RVAE-EM~\cite{wang2024rvae}.
% StoRM and its reference

% Introduce RIR and T60 estimation 

% BUDDy

% \cite{mateljan2003comparison}

% Fourier analyzer

% MLS-based system~\cite{rife1989transfer}

% swept sine system~\cite{farina2000simultaneous}


